Learning Partial Differential Equations in Reproducing Kernel Hilbert Spaces

We propose a new data-driven approach for learning the fundamental solutions (Green's functions) of various linear partial differential equations (PDEs) given sample pairs of input-output functions. Building off the theory of functional linear regression (FLR), we estimate the best-fit Green's function and bias term of the fundamental solution in a reproducing kernel Hilbert space (RKHS) which allows us to regularize their smoothness and impose various structural constraints. We derive a general representer theorem for operator RKHSs to approximate the original infinite-dimensional regression problem by a finite-dimensional one, reducing the search space to a parametric class of Green's functions. In order to study the prediction error of our Green's function estimator, we extend prior results on FLR with scalar outputs to the case with functional outputs. Finally, we demonstrate our method on several linear PDEs including the Poisson, Helmholtz, Schr\"{o}dinger, Fokker-Planck, and heat equation. We highlight its robustness to noise as well as its ability to generalize to new data with varying degrees of smoothness and mesh discretization without any additional training.

==> Learning PDEs in Reproducing Kernel Hilbert Spaces (JMLR)/jmlr_coverletter.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``Learning Partial Differential Equations in Reproducing Kernel Hilbert Spaces'' to the \emph{Journal of Machine Learning Research}.

Our manuscript studies the problem of learning input-output maps (solutions operators) of linear partial differential equations (PDEs) such as the map from a forcing of a PDE to its response. We develop a data-driven, noise robust method that learns such solution operators in a reproducing kernel Hilbert space (RKHS). This leads to a well-posed finite-dimensional optimization problem and further allows us to bound the prediction error of our PDE solution map estimator. We show practical applications of our approach on numerical examples of the Poisson, Helmholtz, Schr\"{o}dinger, Fokker--Planck, and heat equations, where our learned estimators generalize to out-of-distribution functional inputs with varying degrees of smoothness and mesh discretization.

This manuscript is a resubmission of an earlier submission to JMLR from November 14th, 2021. We appreciate the time and effort invested in the review of our manuscript by the action editor and the reviewers from our original submission. In this updated submission, we have taken care to incorporate all of the comments in the feedback left by our reviewers (see attached review rebuttal for point-by-point responses). The new manuscript with the incorporated updates exceeds 50 pages (including appendices and references), as we have put much effort into the theoretical study of our RKHS estimators as well as their implementation and performance on various numerical examples.

We hope that the action editor and reviewers from our first submission to JMLR would be interested in reviewing the updated version of our manuscript. We fully understand if this is not possible, and below we suggest potential action editors and referees for our resubmission.

Action Editors:
\begin{itemize}
    \item Jean-Philippe Vert, Google, France\\(Jean-Philippe.Vert@mines.org)
    \item Lorenzo Rosasco, University of Genova, Italy\\ (lrosasco@mit.edu)
    \item Bernhard Sch\"{o}lkopf, Max Planck Institute for Intelligent Systems, Germany\\(bernhard.schoelkopf@tuebingen.mpg.de)
    \item Michael Mahoney, UC Berkeley, USA\\(mmahoney@stat.berkeley.edu)
    \item John Shawe-Taylor, University College London, UK\\(J.Shawe-Taylor@cs.ucl.ac.uk)
\end{itemize}

Reviewers:
\begin{itemize}
    \item Markus Heinonen, Aalto University, Finland\\(markus.o.heinonen@aalto.fi)
    \item Mauricio A Alvarez, University of Manchester, UK
    \item Marc Peter Deisenroth, University College London, UK
    \item Philipp Hennig, University of T\"{u}bingen, Germany\\(ph@tue.mpg.de)
    \item Ingo Steinwart, University of Stuttgart, Germany\\(ingo.steinwart@mathematik.uni-stuttgart.de)
\end{itemize}

No previous publications by the author overlap with this submission. The submitting author is the sole author of this paper. The author has no conflicts of interest and has not collaborated with any JMLR action editors.

Our submission has the following keywords: Green’s functions, partial differential equations, reproducing kernel Hilbert spaces,
functional linear regression, simultaneous diagonalization.

\bigskip

Sincerely,\\
George Stepaniants

\end{document}








































==> jmlr_coverletter.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``Learning Partial Differential Equations in Reproducing Kernel Hilbert Spaces'' to the \emph{Journal of Machine Learning Research}.

Our manuscript studies the problem of learning input-output maps (solutions operators) of linear partial differential equations (PDEs) such as the map from a forcing of a PDE to its response. We develop a data-driven, noise robust method that learns such solution operators in a reproducing kernel Hilbert space (RKHS). This leads to a well-posed finite-dimensional optimization problem and further allows us to bound the prediction error of our PDE solution map estimator. We show practical applications of our approach on numerical examples of the Poisson, Helmholtz, Schr\"{o}dinger, Fokker--Planck, and heat equations, where our learned estimators generalize to out-of-distribution functional inputs with varying degrees of smoothness and mesh discretization.

This manuscript is a resubmission of an earlier submission to JMLR from November 14th, 2021. We appreciate the time and effort invested in the review of our manuscript by the action editor and the reviewers from our original submission. In this updated submission, we have taken care to incorporate all of the comments in the feedback left by our reviewers (see attached review rebuttal for point-by-point responses). The new manuscript with the incorporated updates exceeds 50 pages (including appendices and references), as we have put much effort into the theoretical study of our RKHS estimators as well as their implementation and performance on various numerical examples.

We hope that the action editor and reviewers from our first submission to JMLR would be interested in reviewing the updated version of our manuscript. We fully understand if this is not possible, and below we suggest potential action editors and referees for our resubmission.

Action Editors:
\begin{itemize}
    \item Jean-Philippe Vert, Google, France\\(Jean-Philippe.Vert@mines.org)
    \item Lorenzo Rosasco, University of Genova, Italy\\ (lrosasco@mit.edu)
    \item Bernhard Sch\"{o}lkopf, Max Planck Institute for Intelligent Systems, Germany\\(bernhard.schoelkopf@tuebingen.mpg.de)
    \item Michael Mahoney, UC Berkeley, USA\\(mmahoney@stat.berkeley.edu)
    \item John Shawe-Taylor, University College London, UK\\(J.Shawe-Taylor@cs.ucl.ac.uk)
\end{itemize}

Reviewers:
\begin{itemize}
    \item Markus Heinonen, Aalto University, Finland\\(markus.o.heinonen@aalto.fi)
    \item Mauricio A Alvarez, University of Manchester, UK
    \item Marc Peter Deisenroth, University College London, UK
    \item Philipp Hennig, University of T\"{u}bingen, Germany\\(ph@tue.mpg.de)
    \item Ingo Steinwart, University of Stuttgart, Germany\\(ingo.steinwart@mathematik.uni-stuttgart.de)
\end{itemize}

No previous publications by the author overlap with this submission. The submitting author is the sole author of this paper. The author has no conflicts of interest and has not collaborated with any JMLR action editors.

Our submission has the following keywords: Green’s functions, partial differential equations, reproducing kernel Hilbert spaces,
functional linear regression, simultaneous diagonalization.

\bigskip

Sincerely,\\
George Stepaniants

\end{document}







































